Stationary subspace analysis of nonstationary covariance processes: eigenstructure description and testing

Stationary subspace analysis (SSA) searches for linear combinations of the components of nonstationary vector time series that are stationary. These linear combinations and their number defne an associated stationary subspace and its dimension. SSA is studied here for zero mean nonstationary covariance processes. We characterize stationary subspaces and their dimensions in terms of eigenvalues and eigenvectors of certain symmetric matrices. This characterization is then used to derive formal statistical tests for estimating dimensions of stationary subspaces. Eigenstructure-based techniques are also proposed to estimate stationary subspaces, without relying on previously used computationally intensive optimization-based methods. Finally, the introduced methodologies are examined on simulated and real data.

==> ssa_descr_old1.tex <==

\section{Constructive descriptions}
\label{s:char}

The observations around (\ref{e:model-vc-ss-2}) and (\ref{e:model-ls-ss-2}) suggest that the stationary subspaces and their dimensions for VC and LS models are related to properties of the symmetric matrices 
\begin{equation}\label{e:models-M}
	M_u = \bar{b}^2(u),\quad M_{u,\lambda} = \bar f(u,\lambda),
\end{equation}
respectively. In this section, we define the matrix quantities of interest and describe them in terms of other commonly used matrix characteristics. 



\subsection{Matrix quantities of interest}
\label{s:char-matrix}

In view of the discussion above, we introduce the following definition. 

\begin{definition}
Let $M$	be a $p\times p$ symmetric matrix. A {\it pseudo dimension} of $M$, denoted $d_0(M)$, is defined as the largest $d_1$ such that
\begin{equation}\label{e:M-pdim}
	C_1 M C_1' = 0,
\end{equation}  
for a $d_1\times p$ matrix $C_1$ with linearly independent rows. A {\it pseudo null space} of $M$, denoted as ${\cal N}_0(M)$, is defined as 
the linear space spanned by the $d_1$ rows of the matrix $C_1$ in (\ref{e:M-pdim}). A row of $C_1$, that is, a row vector $s'$ such that $s'C_1s = 0$ will be 
called a {\it pseudo eigenvector}.  
\end{definition}

In view of (\ref{e:model-vc-ss-2}) and (\ref{e:model-ls-ss-2}), and the notation (\ref{e:M-pdim}), the stationary space and its dimension are then: for VC model,
\begin{equation}\label{e:model-vc-dB1}
	d = d_0(M_u),\quad {\cal B}_1 = {\cal N}_0(M_u),\quad \mbox{for all}\ u, 
\end{equation}
and for LS model, 
\begin{equation}\label{e:model-ls-dB1}
	d = d_0(M_{u,\lambda}),\quad {\cal B}_1 = {\cal N}_0(M_{u,\lambda}),\quad \mbox{for all}\ u, \lambda.
\end{equation}

A word of caution is that ${\cal N}_0(M)$ is not unique in general, as explained in Section \ref{s:char-pnull} below. By writing ${\cal N}_0(M)$, we mean one of the pseudo null spaces.


\subsection{Characterization of pseudo dimension}
\label{s:char-pdim}


We characterize here the pseudo dimension $d_0(M)$ of a symmetric matrix $M$ in terms of more commonly used matrix quantities. The characterization will follow from the next two lemmas. We let 
\begin{equation}\label{e:M-0+-}
	n_0 = \mbox{zero}\{ M \},\quad n_{+} = \mbox{pos}\{M \}, \quad n_{-} = \mbox{neg}\{ M \}
\end{equation}
be the number of zero, positive and negative eigenvalues of $M$. Also, let $\lambda_1 \leq \ldots \leq \lambda_p$ be the ordered eigenvalues of $M$. The zero eigenvalues are denoted $\lambda_{0,i}$,  $i=1,\ldots,n_0$, the positive eigenvalues are denoted $\lambda_{+,i}$, $i=1,\ldots,n_{+}$, and the negative eigenvalues are denoted $\lambda_{-,i}$, $i=1,\ldots,n_-$. 

\begin{lemma}\label{l:rank_claim_1}
Let $M$ be a symmetric matrix. Then, $d_0(M) \leq n_0 +  \min( n_+, n_-)$.
% \begin{equation} \label{e:rank_claim_1}
% \mbox{pdim}\{M\} \leq \mbox{zero}\{ M \} +  \min( \mbox{pos}\{ M \}, \mbox{neg} \{ M \}  ).
% \mbox{pdim}\{M\} \leq n_0 +  \min( n_+, n_-).
% \end{equation}
\end{lemma}

\begin{proof}
By the Poincare Separation Theorem (e.g.\ Magnus and Neudecker \cite{magnus:neudecker:1999}),
\begin{equation*}
\lambda_i \leq \mu_i \leq \lambda_{n-d_1+i}, \quad i=1,\ldots,d_1, 
\end{equation*}
where $\mu_1 \leq \ldots \leq \mu_{d_1}$ are the ordered eigenvalues of $C_1MC_1'$ for any $d_1\times p$ matrix $C_1$ such that $C_1C_1'=I_{d_1}$. Taking $C_1$ as in (\ref{e:M-pdim}) with $d_1=d_0(M)$, we have $C_1MC_1'=0$, and hence 
\begin{equation*}
\lambda_i \leq 0 \leq \lambda_{n-d_1+i}, \quad i=1,\ldots,d_1,
\end{equation*}
which gives the desired result.
\end{proof}


\begin{lemma} \label{l:rank_claim_2}
Let $M$ be a symmetric matrix. Then, $n_0 +  \min( n_+, n_-) \leq d_0(M)$.
% \begin{equation} \label{e:rank_claim_2}
 % \mbox{zero}\{ M \} +  \min( \mbox{pos}\{ M \}, \mbox{neg} \{ M \}  )\leq \mbox{pdim}\{M\} .
 % n_0 +  \min( n_+, n_-) \leq \mbox{pdim}\{M\} .
% \end{equation}
\end{lemma}

\begin{proof}
Let $d_* =  n_0 +  \min( n_+, n_-)$. The proof constructs a $d_* \times p$ matrix $C_1$ such that $C_1MC_1'=0$ and $C_1C_1'=I_{d_*}$, which yields the desired result. By the Schur decomposition (e.g.\ Magnus and Neudecker \cite{magnus:neudecker:1999}), 
\begin{equation}\label{e:M-schur}
S'MS = \mbox{diag}(\lambda_1,\lambda_2,\ldots,\lambda_p),	
\end{equation}
where the columns $s_1, \ldots,s_p$ of $S$ are orthonormal and represent the eigenvectors associated with the eigenvalues $\lambda_1,\ldots,\lambda_p$ of $M$. We need to separate now these eigenvectors into those associated with negative, positive and zero eigenvalues of $M$. Let $s_{0,i}$ be the eigenvectors associated with the zero eigenvalues $\lambda_{0,i}$,  $i=1,\ldots,n_0$, $s_{+,i}$ be the eigenvectors associated with the positive eigenvalues $\lambda_{+,i}$, $i=1,\ldots,n_{+}$, and $s_{-,i}$ be the eigenvectors associated with the negative eigenvalues $\lambda_{-,i}$, $i=1,\ldots,n_-$. Note by (\ref{e:M-schur}) that
\begin{equation}\label{e:M-schur-2}
s_i's_j = \delta_{ij}, \quad  s_i'Ms_j = \delta_{ij} \lambda_{i}.
\end{equation} 

For zero eigenvalues and the corresponding eigenvectors, we have $M s_{0,i} = 0 \cdot s_{0,i}$ and hence 
\begin{equation}\label{e:M-zero-eig}
	s_{0,i}' M s_{0,i} = 0,\quad  i=1,\ldots,n_0.
\end{equation}
Similarly, for the positive and negative eigenvalues, we have 
\begin{eqnarray}
	s_{+,i}' M s_{+,i} & = &  \lambda_{+,i}>0,\quad i=1,\ldots,n_{+}, \label{e:M-pos-eig} \\
	s_{-,i}' M s_{-,i} & = &  \lambda_{-,i}<0,\quad i=1,\ldots,n_{-}. \label{e:M-neg-eig} 
\end{eqnarray}
Let $n_\pm = \min(n_{+},n_{-})$. Then, for some $\alpha_i \in (0,1)$ and $\beta_i = 1-\alpha_i$, we have 
\begin{equation}\label{e:M-posneg-eig=0}
(\alpha_i^{1/2}s_{+,i} + \beta_i^{1/2}s_{-,i})' M (\alpha_i^{1/2}s_{+,i} + \beta_i^{1/2}s_{-,i})
= \alpha_i(s_{+,i}' M s_{+,i}) + \beta_i (s_{-,i}' M s_{-,i}) = 0,
\end{equation}
for $i=1,\ldots,n_\pm$. Set 
\begin{equation}\label{e:M-posneg-eig}
s_{\pm,i} = \frac{\alpha_i^{1/2}s_{+,i} +  \beta_i^{1/2}s_{-,i}}{|| \alpha_i^{1/2}s_{+,i} + \beta_i^{1/2}s_{-,i} ||_2},\quad i=1,\ldots,n_\pm,
\end{equation}
and define a $(n_0+n_\pm) \times p = d_* \times p$ matrix $C_1$ as 
\begin{equation}\label{e:M-posnegzero-C}
C_1' = (s_{0,1}\ \ldots\ s_{0,n_0}\ s_{\pm,1}\ \ldots \ s_{\pm,n_\pm}).
\end{equation}
By using (\ref{e:M-schur-2}), (\ref{e:M-zero-eig}) and (\ref{e:M-posneg-eig=0}), we have $C_1MC_1'=0$. Since $s_i$ are ortonormal and in view of (\ref{e:M-posneg-eig}), we also have 
$C_1C_1' = I_{d_*}$. This concludes the proof.
\end{proof}

The next result follows directly from the two lemmas above.

\begin{corollary}\label{c:rank_claim_3}
Let $M$ be a symmetric matrix. Then,
\begin{equation} \label{e:rank_claim_3}
 % \mbox{zero}\{ M \} +  \min( \mbox{pos}\{ M \}, \mbox{neg} \{ M \}  )\leq \mbox{pdim}\{M\} .
 d_0(M)  = n_0 +  \min( n_+, n_-)= \mbox{\rm zero}\{ M \} +  \min( \mbox{\rm pos}\{ M \}, \mbox{\rm neg} \{ M \}  ).
\end{equation}
\end{corollary}

The first relations in (\ref{e:model-vc-dB1}) and (\ref{e:model-ls-dB1}) can now be reformulated as: for VC model,
\begin{equation}\label{e:model-vc-d-dim}
	d = d_0(M_u) = \mbox{zero}\{ M_u \} +  \min( \mbox{pos}\{ M_u \}, \mbox{neg} \{ M_u \}  ),\quad \mbox{for all}\ u, 
\end{equation}
and for LS model, 
\begin{equation}\label{e:model-ls-d-dim}
	d = d_0( M_{u,\lambda}) = \mbox{zero}\{ M_{u,\lambda} \} +  \min( \mbox{pos}\{ M_{u,\lambda} \}, \mbox{neg} \{ M_{u,\lambda} \}  ),\quad \mbox{for all}\ u, \lambda.
\end{equation} 



\subsection{Characterization of pseudo null space}
\label{s:char-pnull}


A closer examination of the proof of Lemma \ref{l:rank_claim_2} also suggests further insights into the structure of the pseudo null space ${\cal N}_0(M)$. The next auxiliary result describes an element of ${\cal N}_0(M)$. As in the proof of Lemma \ref{l:rank_claim_2}, we let $s_i$ ($s_{0,i}$, $s_{+,i}$ and $s_{-,i}$, resp.) be the orthonormal eigenvectors (associated with zero, positive and negative eigenvalues, resp.) of $M$. We also let $\mbox{null}\{M\}$ denote the null space of the matrix $M$, that is, the linear space spanned by the eigenvectors $s_{0,i}$, $i=1,\ldots,n_0$.

\begin{lemma}\label{l:M-null}
Let $M$ be a symmetric matrix and $w$ be a pseudo eigenvector. Then, 	
\begin{equation}\label{e:M-null-decomp}
	w = w_0 + w_\pm,
\end{equation}
where $w_0\in \mbox{\rm null}\{M\}$ and 
\begin{equation}\label{e:M-null-decomp-1}
	w_\pm = \sum_{i=1}^{n_-} \alpha_{-,i} s_{-,i} + \sum_{i=1}^{n_+} \alpha_{+,i} s_{+,i},
\end{equation}
where $\alpha_{-,i},\alpha_{+,i}\in\RR$ are such that 
\begin{equation}\label{e:M-null-decomp-2}
	\sum_{i=1}^{n_-} \alpha_{-,i}^2 \lambda_{-,i} + \sum_{i=1}^{n_+} \alpha_{+,i}^2 \lambda_{+,i} = 0.
\end{equation}
Vice versa, a vector $w$ expressed through (\ref{e:M-null-decomp})--(\ref{e:M-null-decomp-2}) is a pseudo eigenvector. 
\end{lemma}

\begin{proof}
Any vector $w$ can be expressed as a linear combination of the basis vectors $s_i$ as in (\ref{e:M-null-decomp})--(\ref{e:M-null-decomp-1}). The relation (\ref{e:M-null-decomp-2}) follows since 
$$
0 = w' M w = \sum_{i=1}^{n_0} \alpha_{0,i} s_{0,i}'Ms_{0,i}  + \sum_{i=1}^{n_-} \alpha_{-,i} s_{-,i}'Ms_{-,i} + \sum_{i=1}^{n_+} \alpha_{+,i} s_{+,i}'Ms_{-,i}
$$
$$
= \sum_{i=1}^{n_-} \alpha_{-,i}^2 \lambda_{-,i} + \sum_{i=1}^{n_+} \alpha_{+,i}^2 \lambda_{+,i}. 
$$
The converse statement follows similarly.
\end{proof}


The next result characterizes a pseudo null space ${\cal N}_0(M)$.

\begin{proposition}\label{p:M-null}
Let $M$ be a symmetric matrix and ${\cal N}_0(M)$ be its pseudo null space. Then, 
\begin{equation}\label{e:M-null}
	{\cal N}_0(M) = \mbox{\rm null}\{M\} \oplus {\cal N}_\pm (M),
\end{equation}
where ${\cal N}_\pm (M)$ is a linear space spanned by $\min\{n_0,n_+\}$ orthogornal pseudo vectors expressed as (\ref{e:M-null-decomp-1})--(\ref{e:M-null-decomp-2}). Vice versa, the right-hand side of (\ref{e:M-null}) defines a pseudo null space. Moreover, a pseudo null space is not unique in general.
\end{proposition}

\begin{proof}
The first two statements follow from Lemma \ref{l:M-null} and Corollary \ref{c:rank_claim_3}. The last statement is illustrated in the example given below.
\end{proof}

We next illustrate the results above through a simple but instructive example. See also a subsequent remark.


\begin{example}\label{ex:Mu-analysis}
Consider a VC model with 
\begin{equation}\label{e:ex-b2u}
	b^2(u) = \mbox{diag}(2+\sin(2\pi u),3-\sin(2\pi u),1+\sin(2\pi u)). 
\end{equation}
Then,
\begin{equation}\label{e:ex-b2u-bar}
	\bar b^2(u) = \sin(2\pi u)\cdot \mbox{diag}(1,-1,1). 
\end{equation}
For fixed $u\neq 0,1,1/2$, the eigenvalues of $M := \bar b^2(u)$ are $\sin(2\pi u)\cdot 1$ (of multiplicity 2) and $\sin(2\pi u)\cdot (-1)$. For further illustration, suppose $u\in (0,1/2)$, so that $\sin(2\pi u)>0$. Then, $\lambda_{+,1} = \lambda_{+,2} = \sin(2\pi u)\cdot 1$, $\lambda_{-,1} = \sin(2\pi u)\cdot (-1)$ and $n_+=2$, $n_-=1$, $n_0=0$. By Corollary \ref{c:rank_claim_3}, $d_0(M) = 0 + \min\{1,2\} =1$. The corresponding eigenvectors are $s_{+,1}= (1,\ 0,\ 0)'$, $s_{+,2}= (0,\ 0,\ 1)'$ and $s_{-,1}= (0\ 1\ 0)'$. By Proposition \ref{p:M-null}, a pseudo null space of $M$ can be expressed as
$$
{\cal N}_0(M) = \mbox{lin}\{ \alpha_{-,1} s_{-,1} + \alpha_{+,1} s_{+,1} + \alpha_{+,2} s_{+,2} \}
$$
such that 
$$
-\alpha_{-,1}^2 + \alpha_{+,1}^2 + \alpha_{+,2}^2  = 0
$$
and $\alpha_{-,1}^2 + \alpha_{+,1}^2 + \alpha_{+,2}^2=1$ for the norm to be $1$, where ``lin'' indicates a linear span. The latter two expressions yield $\alpha_{-,1} = (\alpha_{+,1}^2 + \alpha_{+,2}^2)^{1/2}$ (after choosing a positive sign for the square root) and $\alpha_{+,1}^2 + \alpha_{+,2}^2=1/2$. This further yields $\alpha:= \alpha_{+,1}\in [1/\sqrt{2},-1/\sqrt{2}]$, $\alpha_{+,2} = \pm (1/2 - \alpha^2)^{1/2}$ and $\alpha_{-,1} = 1/\sqrt{2}$. Thus, a pseudo null space can also be expressed as
\begin{equation}\label{e:ex-null}
	{\cal N}_0(M) =  \mbox{lin}\{ (1/\sqrt{2}) s_{-,1} + \alpha s_{+,1} \pm (1/2 - \alpha^2)^{1/2} s_{+,2} \} =  \mbox{lin}\{ (\alpha,\ 1/\sqrt{2},\ \pm (1/2 - \alpha^2)^{1/2})' \},
\end{equation}
where $\alpha \in [1/\sqrt{2},-1/\sqrt{2}]$. Note that these spaces (vectors) are generally different for different $\alpha$'s. For example, for $\alpha=0$, 
\begin{equation}\label{e:ex-null-1}
	{\cal N}_0(M) =  \mbox{lin}\{ (0,\ 1/\sqrt{2},\ 1/\sqrt{2})' \} = \mbox{lin}\{ (0,\ 1,\ 1)' \} 
\end{equation}
and for $\alpha=1/\sqrt{2}$, 
\begin{equation}\label{e:ex-null-2}
	{\cal N}_0(M) =  \mbox{lin}\{ (1/\sqrt{2},\ 1/\sqrt{2},\ 0)' \} = \mbox{lin}\{ (1,\ 1,\ 0)' \} .
\end{equation}
\end{example}


\begin{remark}\label{r:ex:Mu-analysis}
The fact that a pseudo null space in Example \ref{ex:Mu-analysis} is not unique should not be surprising from the following perspective. Let $X_t = (X_{1,t},X_{2,t},X_{3,t})'$ be a $3$-variate process following VC model with (\ref{e:ex-b2u}). The pseudo eigenvectors $w_1 = (0,\ 1,\ 1)'$ in (\ref{e:ex-null-1}) and $w_2 = (1,\ 1,\ 0)'$ in (\ref{e:ex-null-2}) can be checked easily to be such that $w_1'X_t$ and $w_2'X_t$ are stationary. 

It is also interesting and important to note here that the stationary dimension for this model is {\it not} $2$. For example, note that while $w_1'X_t$ and $w_2'X_t$ are indeed stationary, the $2$-variate process $(w_1'X_t, w_2'X_t)'$ is {\it not} stationary. Indeed, this is the case since e.g.\ $\EE (w_1'X_t) (w_2'X_t)=\EE(X_{2,t}+X_{3,t})(X_{1,t}+X_{2,t})=\EE X_{2,t}^2=3-\sin(2\pi u)$.
\end{remark}



==> ssa_dimen_old1.tex <==

\section{Inference of dimension}
\label{s:inf-dimens}


...

\subsection{Local pseudo dimension test}
\label{s:inf-dimens-local}


A pseudo dimension $d_0(M)$ of a symmetric matrix $M$ could be tested having a suitable estimator $\widehat M$ of $M$, by adapting the matrix rank tests found in Donald et al.\ \cite{donald:2007rank}. We shall first describe how this can be achieved for general $M$ under suitable assumptions, and then apply the results to VC and LS models.

As in Donald et al.\ \cite{donald:2007rank}, Assumption (A), assume that there is an estimator $\widehat M = \widehat M(N)$ of $M$, depending on some paramater $N$ tending to infinity (e.g.\ the sample size), such that
\begin{equation}\label{e:M-loctest-ass}
	\sqrt{a_N} F(\widehat M - M) F' \stackrel{d}{\to} {\cal Z}_p,
\end{equation}
where $a_N\to \infty$, $F$ is a non-singular $p\times p$ matrix and $ {\cal Z}_p$ is a symmetric $p\times p$ matrix having independent normal entries with variance $1$ on the diagonal and variance $1/2$ off the diagonal. Suppose also that $F$ can be estimated consistently through $\widehat F$, that is, $\widehat F\to_p F$.

We now turn to developing a test for $d_0(M) = n_0 + \min\{n_+,n_-\}$. Since $n_0 = \mbox{zero}\{M\}$ is equal to $p - \mbox{rk}(M)$, where $\mbox{rk}(M)$ is the rank of $M$, we can test directly for $n_0$ by using the MINCHI2 test of Donald et al.\ \cite{donald:2007rank}, Section 4.4.  Let $0 \leq \widehat \gamma_{2,1}\leq \ldots \leq \widehat \gamma_{2,p}$ be the ordered eigenvalues of $(\widehat M \widehat F'\widehat F)^2$. For $r=0,\ldots,p$, consider the test statistic
\begin{equation}\label{e:M-loctest-minchi2}
	\widehat \xi(r) = a_N \sum_{i=1}^{r} \widehat \gamma_{2,i}.
\end{equation}  
The following result reformulates Theorem 4.7 in Donald et al.\ \cite{donald:2007rank} for our purposes here.

\begin{theorem}\label{t:M-loctest-n0}
Suppose that the assumption (\ref{e:M-loctest-ass}) holds. Then, under $H_0:n_0=r$,
\begin{equation}\label{2:M-loctest-n0-1}
	\widehat \xi(r) \stackrel{d}{\to} \chi^2 ( r(r+1)/2 )
\end{equation}
and under $H_0:n_0<r$,
\begin{equation}\label{2:M-loctest-n0-2}
	\widehat \xi(r) \stackrel{p}{\to} +\infty.
\end{equation}
\end{theorem}

The theorem can be used to test for $n_0$ in a standard way sequentially, namely, testing for $H_0:n_0=r$ starting with $r=p$ and subsequently decreasing $r$ by $1$ till the null hypothesis is not rejected. Let $\widehat n_0$ be the resulting estimator, which is consistent for $n_0$ under a suitable choice of critical values in the sequential testing.

Let now $\widehat \gamma_1\leq \ldots \leq \widehat \gamma_p$ be the ordered eigenvalues of $\widehat M \widehat F'\widehat F$ or $\widehat F\widehat M \widehat F'$. Note that $(\widehat \gamma_i)^2 = \widehat \gamma_{2,j(i)}$. It is then natural to estimate the number of negative and positive eigenvalues of $F M F'$ as
\begin{equation}\label{e:M-loctest-n-}
	\widehat n_- = \# \{i: \widehat \gamma_i<0,\quad (\widehat \gamma_i)^2 = \widehat \gamma_{2,k},\quad \mbox{for some}\ k = \widehat n_0+1,\ldots,p\}
\end{equation}
and 
\begin{equation}\label{e:M-loctest-n+}
	\widehat n_+ = \# \{i: \widehat \gamma_i>0,\quad (\widehat \gamma_i)^2 = \widehat \gamma_{2,k},\quad \mbox{for some}\ k = \widehat n_0+1,\ldots,p\}.
\end{equation}
These will consistently estimate the desired quantities since ... It remains to note that $d_0(M) = d_0(FMF')$, so that a natural estimator for $d_0(M)$ is 
\begin{equation}\label{e:M-loctest-d0}
	\widehat d_0(M) = \widehat n_0 + \min\{\widehat n_+,\widehat n_-\}.
\end{equation}


\smallskip

{\bf VC model:} The matrix $M(u)$ of interest for this model can be estimated as
\begin{equation}\label{e:model-vc-Mu-estim}
	\widehat M(u) = \widehat{b}^2(u) -  \widehat{\bar{b}^2} =  \frac{1}{T}\sum_{t=1}^{T}X_tX_t'K_h\Big(u - \frac{t}{T}\Big) - \frac{1}{T}\sum_{t=1}^{T}X_tX_t',
\end{equation}
where $K_h(u) = h^{-1}K(h^{-1}u)$, $K(\cdot)$ is a kernel function and $h$ denotes the bandwidth. The next result shows that, under suitable assumptions, the estimator $\widehat M(u)$ is asymptotically normal for $M(u)$ in the sense of (\ref{e:M-loctest-ass}).

\begin{proposition}\label{p:M-loctest-vc-an}
...
\end{proposition}


\smallskip

{\bf LS model:} ...


\begin{proposition}\label{p:M-loctest-ls-an}
...
\end{proposition}


\subsection{Global pseudo dimension test}
\label{s:inf-dimens-global}


==> ssa_dimen_old2.tex <==

\section{Inference of pseudo dimension}
\label{s:inf-dimens}

According to (\ref{e:model-vc-d-dim})--(\ref{e:model-vc-d-dim-2}), the dimension of a stationary subspace of the VC model is the pseudo dimension $d(M_u)$ of the matrix $M_u$ in (\ref{e:models-M}), assuming it is the same across $u$, which can further be expressed in terms of $d_{0,u}$, $d_{+,u}$ and $d_{-,u}$. We are interested here in the statistical testing for $d_{0,u}$, $d_{+,u}$, $d_{-,u}$ and hence also for $d(M_u)$. We consider below two types of tests: local (that is, for fixed $u$) and global (that is, for an interval of $u$). Though it is the global test which is most relevant for (\ref{e:model-vc-d-dim}) (which is an expression for the interval of $u$), we consider the local test since its statistic forms the basis of the global test and because of independent interest.


For statistical inference, we obviously need an estimator for the matrix $M_u$. It is set naturally as
\begin{equation}\label{e:model-vc-Mu-estim}
	\widehat M_u = \widehat{A}^2(u) -  \widehat{\overline{A}}^2 :=  \frac{1}{T}\sum_{t=1}^{T}X_tX_t'K_h\Big(u - \frac{t}{T}\Big) - \frac{1}{T}\sum_{t=1}^{T}X_tX_t',
\end{equation}
where $K_h(u) = h^{-1}K(h^{-1}u)$, $K(\cdot)$ is a kernel function and $h$ denotes the bandwidth. A kernel is a symmetric function which integrates to $1$, with further regularity assumptions possibly made as well. In simulations and data application, we work with the triangle kernel $K(u) = 1-|u|$ if $|u|<1$ and $0$, otherwise, and the Epanechnikov kernel $K(u)=3(1-u^2)/4$ if $|u|<1$ and $0$, otherwise. 


\subsection{Local pseudo dimension test}
\label{s:inf-dimens-local}


In this section, $u$ is supposed to be fixed. A pseudo dimension $d(M_u)$ of a symmetric matrix $M_u$ could be tested by adapting the matrix rank tests found in \citet{donald:2007rank}. For this, we need an asymptotic normality result for the estimator $\widehat M_u$, which is stated next. We let $\mu_4 = \EE(Z_{i,t}-1)^4$, which can be estimated through
\begin{equation}\label{e:est-mu4}
	\widehat \mu_4 = \frac{1}{Tp} \sum_{i=1}^p\sum_{t=1}^T \Big( (\widehat A(\frac{t}{T})^{-1} X_t)_i^4 - 1\Big).
\end{equation}


\begin{proposition}\label{p:M-loctest-vc-an}
Suppose that the assumptions for the proposition stated in Appendix \ref{s:proofs} hold, in particular, $T\to\infty$, $h\to 0$ so that $Th\to\infty$  and $Th^3\to 0$. Then, we have 
\begin{equation}\label{e:M-loctest-vc-an}
	\frac{\sqrt{Th}}{\|K\|_2 \mu_4^{1/2}} A(u)^{-1} \Big( \widehat M_u - M_u \Big) A(u)^{-1} \stackrel{d}{\to} {\cal Z}_p,
\end{equation}
where $\|K\|_2^2 = \int_\RR K(v)^2 dv$, and ${\cal Z}_p$ is a symmetric $p\times p$ matrix having independent normal entries with variance $1$ on the diagonal and variance $1/\mu_4$ off the diagonal. Moreover, $\widehat{A}^2(u) \to_p A^2(u)$ and $\widehat \mu_4 \to_p \mu_4$.
\end{proposition}


Note that the asymptotic normality result (\ref{e:M-loctest-vc-an}) can be expressed as
\begin{equation}\label{e:M-loctest-ass}
	a_T F_u(\widehat M_u - M_u) F_u' \stackrel{d}{\to} {\cal Z}_p,
\end{equation}
where $a_T=\sqrt{Th}$ and $\widehat F_u\to_p F_u$ with $\widehat F_u = \widehat{A}(u)^{-1}/(\|K\|_2 \widehat \mu_4^{1/2})^{1/2}$. The convergence (\ref{e:M-loctest-ass}) is the setting for the matrix rank tests considered in \cite{donald:2007rank}, with one small difference that plays little role as noted in the proof of Corollary \ref{c:M-loctest-n0}. We explain next how the results of \cite{donald:2007rank} can be adapted to test for $d_{0,u}$, $d_{+,u}$, $d_{-,u}$ and hence also 
for $d(M_u)$.  

We first look at the inference about $d_{0,u}$. Since $d_{0,u}$ is equal to $p - \mbox{rk}(M_u)$, where $\mbox{rk}(M_u)$ is the rank of $M_u$, we can test directly for $d_{0,u}$ by using the MINCHI2 test of \citet{donald:2007rank}, Section 4.4.  Let $0 \leq \widehat \gamma_{2,1,u}\leq \ldots \leq \widehat \gamma_{2,p,u}$ be the ordered eigenvalues of $(\widehat M_u \widehat F_u'\widehat F_u)^2$. For $r=0,\ldots,p$, consider the test statistic
\begin{equation}\label{e:M-loctest-minchi2}
	\widehat \xi_u(r) = a_T^2 \sum_{i=1}^{r} \widehat \gamma_{2,i,u} = Th  \sum_{i=1}^{r} \widehat \gamma_{2,i,u}.
\end{equation}  
Its asymptotics is described in the following result.

\begin{corollary}\label{c:M-loctest-n0}
Suppose that the assumptions of Proposition \ref{p:M-loctest-vc-an} hold. Then, under $H_0:d_{0,u}=r$,
\begin{equation}\label{2:M-loctest-n0-1}
	\widehat \xi_u(r) \stackrel{d}{\to} \chi^2 ( r(r+1)/2 )
\end{equation}
and under $H_1:d_{0,u}<r$,
\begin{equation}\label{2:M-loctest-n0-2}
	\widehat \xi_u(r) \stackrel{p}{\to} +\infty.
\end{equation}
\end{corollary}

\begin{proof}
The result follows from Theorem 4.7 in \citet{donald:2007rank}. Note that the variance in the off-diagonal of the matrix ${\cal Z}_p$ in (\ref{e:M-loctest-ass}) plays no role in the derivation of the theorem, since the argument is based on a trace and hence only on the variance on the diagonal. 
\end{proof}



The corollary can be used to test for $d_{0,u}$ in a standard way sequentially, namely, testing for $H_0:d_{0,u}=r$ starting with $r=p$ and subsequently decreasing $r$ by $1$ till the null hypothesis is not rejected. Let $\widehat d_{0,u}$ be the resulting estimator, which is consistent for $d_{0,u}$ under a suitable choice of critical values in the sequential testing as the following result states.


\begin{corollary}\label{c:M-loctest-n0-2}
Suppose that the assumptions of Proposition \ref{p:M-loctest-vc-an} hold. Let $\widehat d_{0,u}$ be the estimator of $d_{0,u}$ defined above through the sequential testing procedure when using a significance level $\alpha=\alpha_T$ in testing. If $\alpha_T\to 0$ and $(-\log \alpha_T)/Th\to 0$, then $\widehat d_{0,u}\to_p d_{0,u}$. 
\end{corollary}

\begin{proof}
The result can be proved as e.g.\ Theorem 4.3 in \citet{fortuna:2008local}.
\end{proof}


We now turn to inference of $d_{+,u}$ and $d_{-,u}$. Let $\widehat \gamma_{1,u}\leq \ldots \leq \widehat \gamma_{p,u}$ be the ordered eigenvalues of $\widehat M_u \widehat F_u'\widehat F_u$ or $\widehat F_u\widehat M_u \widehat F_u'$. Note that $(\widehat \gamma_{i,u})^2 = \widehat \gamma_{2,j(i),u}$ for some $j(i)$. It is then natural to estimate the number of positive and negative eigenvalues of $F_u M_u F_u'$ (or, equivalently, $M_u$) as
\begin{equation}\label{e:M-loctest-n+-}
	\widehat d_{\pm,u} = \# \{i: \widehat \gamma_{i,u}\gtrless 0,\quad (\widehat \gamma_{i,u})^2 = \widehat \gamma_{2,k,u},\quad \mbox{for some}\ k = \widehat d_{0,u}+1,\ldots,p\}.
\end{equation}
% \begin{equation}\label{e:M-loctest-n+}
% 	\widehat d_{+,u} = \# \{i: \widehat \gamma_{i,u}>0,\quad (\widehat \gamma_{i,u})^2 = \widehat \gamma_{2,k,u},\quad \mbox{for some}\ k = \widehat d_{0,u}+1,\ldots,p\}
% \end{equation}
% and
% \begin{equation}\label{e:M-loctest-n-}
% 	\widehat d_{-,u} = \# \{i: \widehat \gamma_{i,u}<0,\quad (\widehat \gamma_{i,u})^2 = \widehat \gamma_{2,k,u},\quad \mbox{for some}\ k = \widehat d_{0,u}+1,\ldots,p\}.
% \end{equation}

\begin{corollary}\label{c:M-loctest-npm}
Under the assumptions of Corollary \ref{c:M-loctest-n0-2}, we have $\widehat d_{+,u}\to_p d_{+,u}$ and $\widehat d_{-,u}\to_p d_{-,u}$. 
\end{corollary}

\begin{proof}
...
\end{proof}


Finally, a natural estimator for $d(M_u)$ is 
\begin{equation}\label{e:M-loctest-d0}
	\widehat d(M_u) = \widehat d_{0,u} + \min(\widehat d_{+,u},\widehat d_{-,u}).
\end{equation}
Corollaries \ref{c:M-loctest-n0-2}--\ref{c:M-loctest-npm} imply the consistency of this estimator, which is the main result of this section.

\begin{theorem}\label{t:M-loctest-}
Under the assumptions of Corollary \ref{c:M-loctest-n0-2}, we have $\widehat d(M_u)\to_p d(M_u)$. 
\end{theorem}



\subsection{Global pseudo dimension test}
\label{s:inf-dimens-global}


In the previous section, we considered testing about $d_{0,u}$, $d_{+,u}$, $d_{-,u}$ and $d(M_u)$ for fixed $u$. The relation (\ref{e:model-vc-d-dim}) of interest, however, concerns these quantities for $u\in(0,1]$. We would thus like to be able to make inference ``globally,'' that is, for an interval of $u$. Since our approach to $d(M_u)$ goes through $d_{0,u}$, $d_{+,u}$ and $d_{-,u}$, we shall make inference about these quantities first. To deal with the possibility that these quantities might differ across $u\in(0,1]$, we shall work under the assumption that
\begin{equation}\label{e:global-equal}
	d_{0,u} \equiv d_0,\quad d_{+,u} \equiv d_+,\quad d_{-,u} \equiv d_-,\quad u\in {\cal H}\subset (0,1],
\end{equation} 
for each ${\cal H} = {\cal H}_k = ((k-1)/K,k/K]$ from a partition $\sum_{k=1}^K {\cal H}_k = (0,1]$ with some $K\geq 1$. The equivalence signs in (\ref{e:global-equal}) just refers to the fact that the corresponding quantities do not depend on $u\in {\cal H}$.

We shall develop a global pseudo dimension test about $d_0$, $d_+$ and $d_-$ in (\ref{e:global-equal}) for fixed ${\cal H}$, with specific alternatives to (\ref{e:global-equal}) in mind. In practice, these tests will be examined across refined partitions, starting with $K=1$, then $K=2$, etc. See Sections \ref{s:simulation} and \ref{s:application} for illustrations and further discussion.   


We first focus on inference about $d_0$ in (\ref{e:global-equal}). Our global test will be based on the quantity $\int_{\cal H} \widehat \xi_u(r) du$, where $\widehat \xi_u(r)$ is the statistic (\ref{e:M-loctest-minchi2}) used in the local pseudo dimension test. Its asymptotics is described in the next result, which also defines the global statistic $\widehat \xi(r)$. Recall the notation $\mu_4 = \EE (Z_{t,i}-1)^4$ and its estimator $\widehat \mu_4$ defined in (\ref{e:est-mu4}). We also let $|{\cal H}|$ be the length of the interval ${\cal H}$ and $\overline K(u) = \int_\RR K(v) K(u-v) dv$ be the so-called convolution kernel.


\begin{proposition}\label{p:global-an}
Suppose that the assumptions for the proposition stated in Appendix \ref{s:proofs} hold, in particular, ... Then, under $H_0: d_{0,u}\equiv r$ for all $u\in {\cal H}$, 
\begin{equation}\label{e:global-an-1}
	\widehat \xi(r) := \widehat \xi(r; {\cal H}) := \frac{\int_{\cal H} \widehat \xi_u(r) du - |{\cal H}| \frac{r(\widehat \mu_4+r-1)}{\widehat \mu_4}}{\sqrt{h \frac{\|\overline K\|_2^2}{\|K\|_2^4} \frac{2(r\widehat \mu_4^2+2r(r-1))}{\widehat \mu_4^2} |{\cal H}|}} \stackrel{d}{\to} {\cal N}(0,1)
\end{equation}
and under $H_0: d_{0,u}< r$ for some $u\in {\cal H}$, 
\begin{equation}\label{e:global-an-2}
	\widehat \xi(r) \stackrel{p}{\to} \infty.
\end{equation}
\end{proposition}

The proof of the proposition can be found in Appendix \ref{s:proofs}, and follows the approach taken in \citet{donald:2011local}.


\begin{remark}\label{r:global-invariance} 
We note the following natural invariance property of the global test statistic $\widehat \xi(r; {\cal H})$. For ${\cal H}=(0,c]$ with $0<c<1$, we expect the corresponding test statistic $\widehat \xi(r; (0,c])$ to be related to the case ${\cal H}=(0,1]$ and its statistic $\widehat \xi(r; (0,1])$. Indeed, note that 
$$
\int_0^c \widehat \xi_u(r) du = c \int_0^1 \widehat \xi_{cv}(r) dv
$$
where 
$$
\widehat \xi_{cv}(r) = Th \sum_{i=1}^r \widehat \gamma_{2,i}(cv)
$$
and $\widehat \gamma_{2,i}(cv)$ are the eigenvalues of the matrix involving matrices $\widehat M_{cv}$ and $\widehat A^2(cv)$. But note that 
$$
\widehat A^2(cv) = \frac{1}{T} \sum_{t=1}^T X_t X_t' \frac{1}{h} K\Big( \frac{cv - t/T}{h} \Big) \approx \frac{1}{Tc} \sum_{t=1}^{Tc} X_t X_t' \frac{1}{h/c} K\Big( \frac{v - t/(Tc)}{h/c} \Big) =: \widehat A^2_{Tc,h/c}(v), 
$$
where we added subscripts in the last notation to indicate the sample size and the bandwidth. Similarly, with the analogous use of subscripts, $\widehat M_{cv} \approx \widehat M_{Tc,h/c,v}$ -- here, the approximation 
$$
\widehat{\overline{A}}^2 = \frac{1}{T}\sum_{t=1}^{T}X_tX_t' \approx \frac{1}{Tc}\sum_{t=1}^{Tc}X_tX_t' =: \widehat{\overline{A}}_{Tc}^2
$$
is ``justified'' since this term contributes to the asymptotics in Propositions \ref{p:M-loctest-vc-an} and \ref{p:global-an} through the mean. Thus, we effectively have 
$$
\widehat \xi_{cv}(r) \approx \widehat \xi_{Tc,h/c,v}(r). 
$$ 
Note further that $|(0,c]| = c|(0,1]|$ and hence that 
\begin{equation}\label{e:global-invariance}
	\widehat \xi(r; (0,c]) \approx \widehat \xi_{cT,h/c}(r; (0,1]).
\end{equation}
That is, the test statistic $\widehat \xi(r; (0,c])$ has the same structure as that over $(0,1]$ but with the sample size $Tc$ and the bandwidth $h/c$. This of course does not mean that the VC models on $(0,1]$ and $(0,c]$ are equivalent. But if they are, the relation (\ref{e:global-invariance}) provides insight on what to expect when $(0,1]$ is reduced to $(0,c]$, that is, to expect equivalence after adjusting for $T$ and $h$. 
\end{remark}



As for the local tests (see the discussion around Corollary \ref{c:M-loctest-n0-2}), Proposition \ref{p:global-an} can be used to test for $d_0$ sequentially, namely, testing for $H_0:d_0=r$ starting with $r=p$ and subsequently decreasing $r$ by $1$ till the null hypothesis is not rejected. Let $\widehat d_{0}$ be the resulting estimator.


\begin{corollary}\label{c:global-d0-consistency}
Suppose that the assumptions of Proposition \ref{p:global-an} hold. Let $\widehat d_{0}$ be the estimator of $d_{0}$ defined above through the sequential testing procedure when using a significance level $\alpha=\alpha_T$ in testing. If $\alpha_T\to 0$ and $(-\log \alpha_T)/Th\to 0$, then $\widehat d_{0}\to_p d_{0}$. 
\end{corollary}

\begin{proof}
The result can be proved as e.g.\ Theorem 4.3 in \citet{fortuna:2008local}, by noting that the two conditions provided in the statement of the theorem are in fact equivalent.
\end{proof}


We now turn to inference about $d_+$ and $d_-$ in (\ref{e:global-equal}). Recall the definition of the eigenvalues $\widehat \gamma_{i,u}$ preceding (\ref{e:M-loctest-n+-}), whose squares are the eigenvalues $\widehat \gamma_{2,j,u}$ entering the test statistics $\widehat \xi_u(r)$ and $\widehat \xi(r)$. Note that $\widehat d_0$ of the consecutive eigenvalues $\widehat \gamma_{i,u}$ can be thought to be associated with the $d_0$ zero eigenvalues of $M_u$. But we need to estimate the starting index $i$ for these consecutive eigenvalues, from which we can then deduce the numbers $d_\pm$ of positive and negative eigenvalues of $M_u$.  
In the case $\widehat d_0\neq 0$, we thus set
\begin{equation}\label{e:global-stat-d+}
\widehat \zeta(r) = \Big| \int_{\cal H} (\widehat \gamma_{r,u} + \ldots + \widehat \gamma_{r+\widehat d_0-1,u}) du\Big|,\quad r=1,\ldots,p-\widehat d_0+1,
\end{equation}
and estimate this starting index through
\begin{equation}\label{e:global-stat-d+-r}
	\widehat r = \mathop{\rm argmin}_{r=1,\ldots,p-\widehat d_0+1} \widehat \zeta(r).
\end{equation}
(Whenever $r$ does not match the starting index, a larger value of $\widehat \zeta(r)$ is expected, since it will be driven by $\widehat \gamma_{i,u} $ associated with the positive or negative eigenvalues of $M_u$.) This suggests to set further 
\begin{equation}\label{e:global-d+-}
	\widehat d_- = \widehat r - 1,\quad \widehat d_+ = p - \widehat d_0 - \widehat d_-.
\end{equation}


If $\widehat d_0=0$, the preceding argument does not apply and, in fact, the quantity (\ref{e:global-stat-d+}) is not even defined. In this case, we suggest to consider 
\begin{equation}\label{e:global-stat-d+-2}
	\widehat \eta(r) = \Big|\int_{\cal H} (\widehat \gamma_{1,u} + \ldots + \widehat \gamma_{r,u}) du \Big| + \Big|\int_{\cal H} (\widehat \gamma_{r+1,u} + \ldots + \widehat \gamma_{p,u}) du \Big|,\quad r=0,\ldots,p,
\end{equation}
and set 
\begin{equation}\label{e:global-d+-2}
	\widehat d_- =  \mathop{\rm argmax}_{r=0,\ldots,p}\, \widehat \eta(r),\quad \widehat d_+ = p - \widehat d_-. 
\end{equation}
The idea behind these definition is that $\widehat \eta(r)$ can be thought as estimating the respective population quantity $\eta(r) = |\int_{\cal H} (\gamma_{1,u} + \ldots + \gamma_{r,u}) du | + |\int_{\cal H} (\gamma_{r+1,u} + \ldots + \gamma_{p,u}) du |$, where $\gamma_{1,u}\leq \ldots \leq \gamma_{p,u}$ are the ordered eigenvalues of $F_u M_u F_u'$. The number of these eigenvalues that are negative is then the index $r$ for which $\eta(r)$ is largest, motivating (\ref{e:global-stat-d+-2})--(\ref{e:global-d+-2}).


\begin{corollary}\label{c:global-d+--consistency}
Under the assumptions of Corollary \ref{c:global-d0-consistency}, we have $\widehat d_{+}\to_p d_{+}$ and $\widehat d_{-}\to_p d_{-}$. 
\end{corollary}

\begin{proof}
...
\end{proof}


Finally, a natural estimator for $d := d_0 + \min(d_+,d_-)$ is 
\begin{equation}\label{e:global-d}
	\widehat d = \widehat d_{0} + \min(\widehat d_{+},\widehat d_{-}).
\end{equation}
Corollaries \ref{c:global-d0-consistency}--\ref{c:global-d+--consistency} imply the consistency of this estimator, which is the main result of this section.

\begin{theorem}\label{t:global-d}
Under the assumptions of Corollary \ref{c:global-d0-consistency}, we have $\widehat d\to_p d$. 
\end{theorem}








==> ssa_dimen_old3.tex <==

\section{Inference of pseudo dimension}
\label{s:inf-dimens}

According to (\ref{e:model-vc-d-dim})--(\ref{e:model-vc-d-dim-2}), the dimension of a stationary subspace of the VC model is the pseudo dimension $d(M(u))$ of the matrix $M(u)$ in (\ref{e:models-M}), assuming it is the same across $u$, which can further be expressed in terms of $d_0(u)$, $d_+(u)$ and $d_-(u)$. We are interested here in the statistical testing for $d_0(u)$, $d_+(u)$, $d_-(u)$ and hence also for $d(M(u))$. We consider below two types of tests: local (that is, for fixed $u$) and global (that is, for an interval of $u$). Though it is the global test which is most relevant for (\ref{e:model-vc-d-dim}) (which is an expression for the interval of $u$), we consider the local test since its statistic forms the basis of the global test and because of independent interest.


For statistical inference, we obviously need an estimator for the matrix $M(u)$. It is set naturally as
\begin{equation}\label{e:model-vc-Mu-estim}
	\widehat M(u) = \widehat{A}^2(u) -  \widehat{\overline{A}}^2 :=  \frac{1}{T}\sum_{t=1}^{T}X_tX_t'K_h\Big(u - \frac{t}{T}\Big) - \frac{1}{T}\sum_{t=1}^{T}X_tX_t',
\end{equation}
where $K_h(u) = h^{-1}K(h^{-1}u)$, $K(\cdot)$ is a kernel function and $h$ denotes the bandwidth. A kernel is a symmetric function which integrates to $1$, with further regularity assumptions possibly made as well. In simulations and data application, we work with the triangle kernel $K(u) = 1-|u|$ if $|u|<1$ and $0$, otherwise, and the Epanechnikov kernel $K(u)=3(1-u^2)/4$ if $|u|<1$ and $0$, otherwise. 


\subsection{Local pseudo dimension test}
\label{s:inf-dimens-local}


In this section, $u$ is supposed to be fixed. A pseudo dimension $d(M(u))$ of a symmetric matrix $M(u)$ could be tested by adapting the matrix rank tests found in \citet{donald:2007rank}. For this, we need an asymptotic normality result for the estimator $\widehat M(u)$, which is stated next. The proof can be found in Appendix \ref{s:proofs-local}.



\begin{proposition}\label{p:M-loctest-vc-an}
Suppose that the assumptions for the proposition stated in Appendix \ref{s:proofs} hold, in particular, $T\to\infty$, $h\to 0$ so that $Th\to\infty$  and $Th^3\to 0$. Then, we have 
\begin{equation}\label{e:M-loctest-vc-an}
	\frac{\sqrt{Th}}{\|K\|_2 \mu_4^{1/2}} A(u)^{-1} \Big( \widehat M(u) - M(u) \Big) A(u)'^{-1} \stackrel{d}{\to} {\cal Z}_p,
\end{equation}
where $\|K\|_2^2 = \int_\RR K(v)^2 dv$, $\mu_4 = \EE(Y_{i,t}^2-1)^2=\EE Y_{i,t}^4-1$ and ${\cal Z}_p$ is a symmetric $p\times p$ matrix having independent normal entries with variance $1$ on the diagonal and variance $1/\mu_4$ off the diagonal. Moreover, $\widehat{A}^k(u) \to_p A^k(u)$, $k=\pm 1,\pm 2$.
\end{proposition}



Note that the asymptotic normality result (\ref{e:M-loctest-vc-an}) can be expressed as
\begin{equation}\label{e:M-loctest-ass}
	a_T F(u)(\widehat M(u) - M(u)) F(u)' \stackrel{d}{\to} {\cal Z}_p,
\end{equation}
where $a_T=\sqrt{Th}$ and $F(u)=A(u)^{-1}/(\|K\|_2 \mu_4^{1/2})^{1/2}$. Furthermore, by Proposition \ref{p:M-loctest-vc-an}, we have
\begin{equation}\label{e:M-loctest-ass-2}
	\widehat F(u)\to_p F(u)
\end{equation}
with $\widehat F(u) = \widehat{A}(u)^{-1}/(\|K\|_2 \widehat \mu_4^{1/2})^{1/2}$, provided an estimator $\widehat \mu_4$ is consistent for $\mu_4$. For better readibility, construction of consistent estimators $\widehat \mu_4$ is discussed in Appendix \ref{s:proofs-4moment}. Furthermore, if one is willing to assume Gaussianity of $Y_t$, note that $\mu_4=2$ can also be used.


The convergence (\ref{e:M-loctest-ass}) with (\ref{e:M-loctest-ass-2}) is the setting for the matrix rank tests considered in \cite{donald:2007rank}, with one small difference that plays little role as noted in the proof of Corollary \ref{c:M-loctest-n0}. We explain next how the results of \cite{donald:2007rank} can be adapted to test for $d_0(u)$, $d_+(u)$, $d_-(u)$ and hence also 
for $d(M(u))$.  



We first look at the inference about $d_0(u)$. Since $d_0(u)$ is equal to $p - \mbox{rk}(M(u))$, where $\mbox{rk}(M(u))$ is the rank of $M(u)$, we can test directly for $d_0(u)$ by using the MINCHI2 test of \citet{donald:2007rank}, Section 4.4.  Let $0 \leq \widehat \gamma_{2,1}(u)\leq \ldots \leq \widehat \gamma_{2,p}(u)$ be the ordered eigenvalues of $(\widehat M(u) \widehat F(u)'\widehat F(u))^2$. For $r=0,\ldots,p$, consider the test statistic
\begin{equation}\label{e:M-loctest-minchi2}
	\widehat \xi_r(u) = a_T^2 \sum_{i=1}^{r} \widehat \gamma_{2,i}(u) = Th  \sum_{i=1}^{r} \widehat \gamma_{2,i}(u).
\end{equation}  
Its asymptotics is described in the following result.

\begin{corollary}\label{c:M-loctest-n0}
Suppose that the assumptions of Proposition \ref{p:M-loctest-vc-an} hold. Then, under $H_0:d_0(u)=r$,
\begin{equation}\label{2:M-loctest-n0-1}
	\widehat \xi_r(u) \stackrel{d}{\to} \chi^2 ( r(r+1)/2 )
\end{equation}
and under $H_1:d_0(u)<r$,
\begin{equation}\label{2:M-loctest-n0-2}
	\widehat \xi_r(u) \stackrel{p}{\to} +\infty.
\end{equation}
\end{corollary}

\begin{proof}
The result follows from Theorem 4.7 in \citet{donald:2007rank}. Note that the variance in the off-diagonal of the matrix ${\cal Z}_p$ in (\ref{e:M-loctest-ass}) plays no role in the derivation of the theorem, since the argument is based on a trace and hence only on the variance on the diagonal. 
\end{proof}



The corollary can be used to test for $d_0(u)$ in a standard way sequentially, namely, testing for $H_0:d_0(u)=r$ starting with $r=p$ and subsequently decreasing $r$ by $1$ till the null hypothesis is not rejected. Let $\widehat d_0(u)$ be the resulting estimator, which is consistent for $d_0(u)$ under a suitable choice of critical values in the sequential testing as the following result states.


\begin{corollary}\label{c:M-loctest-n0-2}
Suppose that the assumptions of Proposition \ref{p:M-loctest-vc-an} hold. Let $\widehat d_0(u)$ be the estimator of $d_0(u)$ defined above through the sequential testing procedure when using a significance level $\alpha=\alpha_T$ in testing. If $\alpha_T\to 0$ and $(-\log \alpha_T)/Th\to 0$, then $\widehat d_0(u)\to_p d_0(u)$. 
\end{corollary}

\begin{proof}
The result can be proved as e.g.\ Theorem 4.3 in \citet{fortuna:2008local}.
\end{proof}


We now turn to inference of $d_+(u)$ and $d_-(u)$. Let $\widehat \gamma_{1}(u)\leq \ldots \leq \widehat \gamma_{p}(u)$ be the ordered eigenvalues of $\widehat M(u) \widehat F(u)'\widehat F(u)$ or $\widehat F(u)\widehat M(u) \widehat F(u)'$. Note that $(\widehat \gamma_{i}(u))^2 = \widehat \gamma_{2,j(i)}(u)$ for some $j(i)$. It is then natural to estimate the number of positive and negative eigenvalues of $F(u) M(u) F(u)'$ (or, equivalently, $M(u)$) as
\begin{equation}\label{e:M-loctest-n+-}
	\widehat d_{\pm}(u) = \# \{i: \widehat \gamma_{i}(u)\gtrless 0,\quad (\widehat \gamma_{i}(u))^2 = \widehat \gamma_{2,k}(u),\quad \mbox{for some}\ k = \widehat d_0(u)+1,\ldots,p\}.
\end{equation}
% \begin{equation}\label{e:M-loctest-n+}
% 	\widehat d_{+,u} = \# \{i: \widehat \gamma_{i,u}>0,\quad (\widehat \gamma_{i,u})^2 = \widehat \gamma_{2,k,u},\quad \mbox{for some}\ k = \widehat d_{0,u}+1,\ldots,p\}
% \end{equation}
% and
% \begin{equation}\label{e:M-loctest-n-}
% 	\widehat d_{-,u} = \# \{i: \widehat \gamma_{i,u}<0,\quad (\widehat \gamma_{i,u})^2 = \widehat \gamma_{2,k,u},\quad \mbox{for some}\ k = \widehat d_{0,u}+1,\ldots,p\}.
% \end{equation}

\begin{corollary}\label{c:M-loctest-npm}
Under the assumptions of Corollary \ref{c:M-loctest-n0-2}, we have $\widehat d_+(u)\to_p d_+(u)$ and $\widehat d_-(u)\to_p d_-(u)$. 
\end{corollary}

\begin{proof}
Let $0\leq \gamma_{2,1}(u)\leq \ldots\leq \gamma_{2,p}(u)$ be the ordered eigenvalues of $(F(u)M(u)F(u)')^2$ and $\gamma_1(u)\leq \ldots\leq \gamma_p(u)$ be the ordered eigenvalues of $F(u)M(u)F(u)'$. We have $\gamma_{2,j(i)}(u) = (\gamma_i(u))^2$ for some $j(i)$; $\gamma_{2,j}(u)=0$ for $j=1,\ldots,d_0(u)$ and $\gamma_{2,j}(u)>0$ for $j=d_0(u)+1,\ldots,p$; $\gamma_i(u)<0$ for $i=1,\ldots,d_-(u)$, $\gamma_i(u)=0$ for $i=d_-(u)+1,\ldots,d_-(u)+d_0(u)$ and   $\gamma_i(u)>0$ for $i=d_-(u)+d_0(u)+1,\ldots,p$. The stated result now follows from the following two observations. First, by Corollary \ref{c:M-loctest-n0-2}, $\widehat d_0(u)=d_0(u)$ a.s.\ for large enough $T$ (depending on $\omega$ in ``a.s.''). Second, since $(\widehat F(u)\widehat M(u) \widehat F(u)')^k\to_p (F(u)M(u)F(u)')^k$ for $k=1,2$, we have $\widehat \gamma_{2,j}(u)\to_p \gamma_{2,j}(u)$, $j=1,\ldots,p$, and $\widehat \gamma_i(u)\to_p \gamma_i(u)$, $i=1,\ldots,p$. That is, $\widehat d_0(u)=d_0(u)$ ensures that the total number (sum) of positive and negative eigenvalues can be identified by focusing only on   $\widehat \gamma_{2,k}(u) = (\widehat \gamma_{i(k)}(u))^2$ with $k=\widehat d_0(u)+1,\ldots,p$. Because of consistency of $\widehat \gamma_i(u)$, we further expect that $d_-(u)$ will be the number of $\widehat \gamma_{i(k)}(u)$ which are negative (eventually), and similarly for $d_+(u)$. 
\end{proof}


Finally, a natural estimator for $d(M(u))$ is 
\begin{equation}\label{e:M-loctest-d0}
	\widehat d(M(u)) = \widehat d_0(u) + \min(\widehat d_+(u),\widehat d_-(u)).
\end{equation}
Corollaries \ref{c:M-loctest-n0-2}--\ref{c:M-loctest-npm} imply the consistency of this estimator, which is the main result of this section.

\begin{theorem}\label{t:M-loctest-}
Under the assumptions of Corollary \ref{c:M-loctest-n0-2}, we have $\widehat d(M(u))\to_p d(M(u))$. 
\end{theorem}



\subsection{Global pseudo dimension test}
\label{s:inf-dimens-global}


In the previous section, we considered testing about $d_{0,u}$, $d_{+,u}$, $d_{-,u}$ and $d(M_u)$ for fixed $u$. The relation (\ref{e:model-vc-d-dim}) of interest, however, concerns these quantities for $u\in(0,1]$. We would thus like to be able to make inference ``globally,'' that is, for an interval of $u$. Since our approach to $d(M_u)$ goes through $d_{0,u}$, $d_{+,u}$ and $d_{-,u}$, we shall make inference about these quantities first. To deal with the possibility that these quantities might differ across $u\in(0,1]$, we shall work under the assumption that
\begin{equation}\label{e:global-equal}
	d_{0,u} \equiv d_0,\quad d_{+,u} \equiv d_+,\quad d_{-,u} \equiv d_-,\quad u\in {\cal H}\subset (0,1],
\end{equation} 
for each ${\cal H} = {\cal H}_k = ((k-1)/K,k/K]$ from a partition $\sum_{k=1}^K {\cal H}_k = (0,1]$ with some $K\geq 1$. The equivalence signs in (\ref{e:global-equal}) just refers to the fact that the corresponding quantities do not depend on $u\in {\cal H}$.

We shall develop a global pseudo dimension test about $d_0$, $d_+$ and $d_-$ in (\ref{e:global-equal}) for fixed ${\cal H}$, with specific alternatives to (\ref{e:global-equal}) in mind. In practice, these tests will be examined across refined partitions, starting with $K=1$, then $K=2$, etc. See Sections \ref{s:simulation} and \ref{s:application} for illustrations and further discussion.   


We first focus on inference about $d_0$ in (\ref{e:global-equal}). Our global test will be based on the quantity $\int_{\cal H} \widehat \xi_u(r) du$, where $\widehat \xi_u(r)$ is the statistic (\ref{e:M-loctest-minchi2}) used in the local pseudo dimension test. Its asymptotics is described in the next result, which also defines the global statistic $\widehat \xi(r)$. Recall the notation $\mu_4 = \EE (Z_{t,i}-1)^4$ and its estimator $\widehat \mu_4$ defined in (\ref{e:est-mu4}). We also let $|{\cal H}|$ be the length of the interval ${\cal H}$ and $\overline K(u) = \int_\RR K(v) K(u-v) dv$ be the so-called convolution kernel.


\begin{proposition}\label{p:global-an}
Suppose that the assumptions for the proposition stated in Appendix \ref{s:proofs} hold, in particular, ... Then, under $H_0: d_{0,u}\equiv r$ for all $u\in {\cal H}$, 
\begin{equation}\label{e:global-an-1}
	\widehat \xi(r) := \widehat \xi(r; {\cal H}) := \frac{\int_{\cal H} \widehat \xi_u(r) du - |{\cal H}| \frac{r(\widehat \mu_4+r-1)}{\widehat \mu_4}}{\sqrt{h \frac{\|\overline K\|_2^2}{\|K\|_2^4} \frac{2(r\widehat \mu_4^2+2r(r-1))}{\widehat \mu_4^2} |{\cal H}|}} \stackrel{d}{\to} {\cal N}(0,1)
\end{equation}
and under $H_0: d_{0,u}< r$ for some $u\in {\cal H}$, 
\begin{equation}\label{e:global-an-2}
	\widehat \xi(r) \stackrel{p}{\to} \infty.
\end{equation}
\end{proposition}

The proof of the proposition can be found in Appendix \ref{s:proofs}, and follows the approach taken in \citet{donald:2011local}.


\begin{remark}\label{r:global-invariance} 
We note the following natural invariance property of the global test statistic $\widehat \xi(r; {\cal H})$. For ${\cal H}=(0,c]$ with $0<c<1$, we expect the corresponding test statistic $\widehat \xi(r; (0,c])$ to be related to the case ${\cal H}=(0,1]$ and its statistic $\widehat \xi(r; (0,1])$. Indeed, note that 
$$
\int_0^c \widehat \xi_u(r) du = c \int_0^1 \widehat \xi_{cv}(r) dv
$$
where 
$$
\widehat \xi_{cv}(r) = Th \sum_{i=1}^r \widehat \gamma_{2,i}(cv)
$$
and $\widehat \gamma_{2,i}(cv)$ are the eigenvalues of the matrix involving matrices $\widehat M_{cv}$ and $\widehat A^2(cv)$. But note that 
$$
\widehat A^2(cv) = \frac{1}{T} \sum_{t=1}^T X_t X_t' \frac{1}{h} K\Big( \frac{cv - t/T}{h} \Big) \approx \frac{1}{Tc} \sum_{t=1}^{Tc} X_t X_t' \frac{1}{h/c} K\Big( \frac{v - t/(Tc)}{h/c} \Big) =: \widehat A^2_{Tc,h/c}(v), 
$$
where we added subscripts in the last notation to indicate the sample size and the bandwidth. Similarly, with the analogous use of subscripts, $\widehat M_{cv} \approx \widehat M_{Tc,h/c,v}$ -- here, the approximation 
$$
\widehat{\overline{A}}^2 = \frac{1}{T}\sum_{t=1}^{T}X_tX_t' \approx \frac{1}{Tc}\sum_{t=1}^{Tc}X_tX_t' =: \widehat{\overline{A}}_{Tc}^2
$$
is ``justified'' since this term contributes to the asymptotics in Propositions \ref{p:M-loctest-vc-an} and \ref{p:global-an} through the mean. Thus, we effectively have 
$$
\widehat \xi_{cv}(r) \approx \widehat \xi_{Tc,h/c,v}(r). 
$$ 
Note further that $|(0,c]| = c|(0,1]|$ and hence that 
\begin{equation}\label{e:global-invariance}
	\widehat \xi(r; (0,c]) \approx \widehat \xi_{cT,h/c}(r; (0,1]).
\end{equation}
That is, the test statistic $\widehat \xi(r; (0,c])$ has the same structure as that over $(0,1]$ but with the sample size $Tc$ and the bandwidth $h/c$. This of course does not mean that the VC models on $(0,1]$ and $(0,c]$ are equivalent. But if they are, the relation (\ref{e:global-invariance}) provides insight on what to expect when $(0,1]$ is reduced to $(0,c]$, that is, to expect equivalence after adjusting for $T$ and $h$. 
\end{remark}



As for the local tests (see the discussion around Corollary \ref{c:M-loctest-n0-2}), Proposition \ref{p:global-an} can be used to test for $d_0$ sequentially, namely, testing for $H_0:d_0=r$ starting with $r=p$ and subsequently decreasing $r$ by $1$ till the null hypothesis is not rejected. Let $\widehat d_{0}$ be the resulting estimator.


\begin{corollary}\label{c:global-d0-consistency}
Suppose that the assumptions of Proposition \ref{p:global-an} hold. Let $\widehat d_{0}$ be the estimator of $d_{0}$ defined above through the sequential testing procedure when using a significance level $\alpha=\alpha_T$ in testing. If $\alpha_T\to 0$ and $(-\log \alpha_T)/Th\to 0$, then $\widehat d_{0}\to_p d_{0}$. 
\end{corollary}

\begin{proof}
The result can be proved as e.g.\ Theorem 4.3 in \citet{fortuna:2008local}, by noting that the two conditions provided in the statement of the theorem are in fact equivalent.
\end{proof}


We now turn to inference about $d_+$ and $d_-$ in (\ref{e:global-equal}). Recall the definition of the eigenvalues $\widehat \gamma_{i,u}$ preceding (\ref{e:M-loctest-n+-}), whose squares are the eigenvalues $\widehat \gamma_{2,j,u}$ entering the test statistics $\widehat \xi_u(r)$ and $\widehat \xi(r)$. Note that $\widehat d_0$ of the consecutive eigenvalues $\widehat \gamma_{i,u}$ can be thought to be associated with the $d_0$ zero eigenvalues of $M_u$. But we need to estimate the starting index $i$ for these consecutive eigenvalues, from which we can then deduce the numbers $d_\pm$ of positive and negative eigenvalues of $M_u$.  
In the case $\widehat d_0\neq 0$, we thus set
\begin{equation}\label{e:global-stat-d+}
\widehat \zeta(r) = \Big| \int_{\cal H} (\widehat \gamma_{r,u} + \ldots + \widehat \gamma_{r+\widehat d_0-1,u}) du\Big|,\quad r=1,\ldots,p-\widehat d_0+1,
\end{equation}
and estimate this starting index through
\begin{equation}\label{e:global-stat-d+-r}
	\widehat r = \mathop{\rm argmin}_{r=1,\ldots,p-\widehat d_0+1} \widehat \zeta(r).
\end{equation}
(Whenever $r$ does not match the starting index, a larger value of $\widehat \zeta(r)$ is expected, since it will be driven by $\widehat \gamma_{i,u} $ associated with the positive or negative eigenvalues of $M_u$.) This suggests to set further 
\begin{equation}\label{e:global-d+-}
	\widehat d_- = \widehat r - 1,\quad \widehat d_+ = p - \widehat d_0 - \widehat d_-.
\end{equation}


If $\widehat d_0=0$, the preceding argument does not apply and, in fact, the quantity (\ref{e:global-stat-d+}) is not even defined. In this case, we suggest to consider 
\begin{equation}\label{e:global-stat-d+-2}
	\widehat \eta(r) = \Big|\int_{\cal H} (\widehat \gamma_{1,u} + \ldots + \widehat \gamma_{r,u}) du \Big| + \Big|\int_{\cal H} (\widehat \gamma_{r+1,u} + \ldots + \widehat \gamma_{p,u}) du \Big|,\quad r=0,\ldots,p,
\end{equation}
and set 
\begin{equation}\label{e:global-d+-2}
	\widehat d_- =  \mathop{\rm argmax}_{r=0,\ldots,p}\, \widehat \eta(r),\quad \widehat d_+ = p - \widehat d_-. 
\end{equation}
The idea behind these definition is that $\widehat \eta(r)$ can be thought as estimating the respective population quantity $\eta(r) = |\int_{\cal H} (\gamma_{1,u} + \ldots + \gamma_{r,u}) du | + |\int_{\cal H} (\gamma_{r+1,u} + \ldots + \gamma_{p,u}) du |$, where $\gamma_{1,u}\leq \ldots \leq \gamma_{p,u}$ are the ordered eigenvalues of $F_u M_u F_u'$. The number of these eigenvalues that are negative is then the index $r$ for which $\eta(r)$ is largest, motivating (\ref{e:global-stat-d+-2})--(\ref{e:global-d+-2}).


\begin{corollary}\label{c:global-d+--consistency}
Under the assumptions of Corollary \ref{c:global-d0-consistency}, we have $\widehat d_{+}\to_p d_{+}$ and $\widehat d_{-}\to_p d_{-}$. 
\end{corollary}

\begin{proof}
...
\end{proof}


Finally, a natural estimator for $d := d_0 + \min(d_+,d_-)$ is 
\begin{equation}\label{e:global-d}
	\widehat d = \widehat d_{0} + \min(\widehat d_{+},\widehat d_{-}).
\end{equation}
Corollaries \ref{c:global-d0-consistency}--\ref{c:global-d+--consistency} imply the consistency of this estimator, which is the main result of this section.

\begin{theorem}\label{t:global-d}
Under the assumptions of Corollary \ref{c:global-d0-consistency}, we have $\widehat d\to_p d$. 
\end{theorem}








==> ssa_models_old1.tex <==

\section{Models of interest and their stationary subspaces}
\label{s:models}

We focus throughout this work on two models of nonstationary processes: a varying covariance or VC model (Section \ref{s:models-vc}) and a locally stationary or LS model (Section \ref{s:models-ls}). As noted in Section \ref{s:intro}, we assume that these models have zero mean. VC model, which has no stochastic temporal dependence, is in the spirit of the first nonstationary models considered in the SSA literture ( \cite{von:2009finding}). LS model, on the other hand, allows for stochastic temporal dependence (similarly to \cite{sundararajan:2017}).


\subsection{VC model}
\label{s:models-vc}

In this model, the observed $p$-variate time series $X_t$ is given by
\begin{equation} \label{e:model-vc}
X_{t} =  b\Big(\frac{t}{T}\Big) Z_t,\quad t=1,\ldots,T,
\end{equation}
where $  b:[0,1] \rightarrow \mathbb{R}^{p \times p}$ is a smoothly varying matrix-valued function and  $Z_t$ are i.i.d.\ random vectors with $\EE(Z_t)=0$ and $\EE(Z_tZ_t') = I_p$. {\bf Taking the first few rows of $b()$ to be constant leads to the setup in (1).} Further technical assumptions can be found below.

The existence of a stationary subspace for this model can be formulated as: there is a $d\times p$ matrix $B_1$ such that $B_1B_1' = I_d$ and
\begin{equation}\label{e:model-vc-ss}
	B_1 b^2(u) B_1' = \Sigma,
\end{equation}
where  $b^2(u) = b(u) b(u)'$ and $\Sigma$ does not depend on $u$. The condition (\ref{e:model-vc-ss}) is equivalent to
\begin{equation}\label{e:model-vc-ss-2}
	B_1 \bar{b}^2(u)  B_1' = B_1 (b^2(u)  -  \bar{b}^2) B_1'  = 0,
\end{equation}
where $\bar{b}^2 = \int_0^1 b^2(u) du$. Note that the $p \times p$ matrix $\bar{b}^2(u)$ is symmetric. As before, the dimension $d$ of a stationary subspace is the largest $d$ for which (\ref{e:model-vc-ss-2}) holds.



\subsection{LS model}
\label{s:models-ls}

For this model, we consider a $p$-variate locally stationary (LS) time series expressed in the spectral domain as
\begin{equation}\label{e:model-ls}
	X_{t} = \int_{-\pi}^\pi e^{i\lambda t} A^0_{t,T}(\lambda) Z(d\lambda),\quad t=1,\ldots, T,
\end{equation}
where $A^0_{t,T}(\lambda)$ is complex-valued and $p\times p$, and $Z(d\lambda)$ is a suitable $p\times 1$ complex-valued random measure. This follows the developments in the univariate case $p=1$ found in  \cite{dahlhaus:1997fitting}. Following  \cite{dahlhaus:1997fitting}, one basic assumption is to require that
\begin{equation}\label{e:model-ls-assumpt}
	A^0_{t,T}(\lambda) \approx A\Big(\frac{t}{T},\lambda\Big),
\end{equation}
for a suitable matrix-valued function $A(u,\lambda)$. Further technical assumptions can be found below. The quantity
\begin{equation}\label{e:model-ls-density}
f(u,\lambda) = A(u,\lambda)A(u,\lambda)^*
\end{equation}
is called the time varying spectral density matrix of the model.

The existence of a stationary subspace could then be formulated as: there is a $d\times p$ matrix $B_1$ (with linearly independent rows) such that $B_1B_1' = I_d$ and
\begin{equation}\label{e:model-ls-ss}
	B_1 f(u,\lambda) B_1' = G(\lambda),
\end{equation}
where the matrix function $G(\lambda)$ does not depend on $u$. This condition is equivalent to
\begin{equation}\label{e:model-ls-ss-2}
	B_1 \bar f(u,\lambda) B_1' = B_1 ( f(u,\lambda) - \bar f(\lambda)) B_1' = 0,
\end{equation}
where $\bar f(\lambda)=\int_0^1 f(u,\lambda) du$. Again, the $p\times p$ matrix is $\bar f(u,\lambda)$ symmetric. The dimension $d$ of a stationary subspace is the largest $d$ for which (\ref{e:model-ls-ss-2}) holds.


==> ssa_models_old2.tex <==

\section{Model of interest and its stationary subspace}
\label{s:models}

We focus throughout this work on a varying covariance (VC) model. The VC model, which has no stochastic temporal dependence, is in the spirit of the first models considered in the SSA literature (\citet{von:2009finding}). More specifically, the observed $p$--variate time series $X_t$ is given by
\begin{equation} \label{e:model-vc}
X_{t} =  A\Big(\frac{t}{T}\Big) Y_t,\quad t=1,\ldots,T,
\end{equation}
where $ A:(0,1] \rightarrow \mathbb{R}^{p \times p}$ is a smoothly varying matrix-valued function and  $Y_t$ are i.i.d.\ random vectors with i.i.d.\ entries, $\EE(Y_t)=0$ and $\EE(Y_t Y_t') = I_p$. 
% {\bf Taking the first few rows of $b()$ to be constant leads to the setup in (1).}
Further technical assumptions can be found below.

\begin{definition}
\textbf{(a):} We say there exists a (second-order) \textit{stationary subspace} of dimension $d$ for model \eqref{e:model-vc} if $d$ is the largest integer in $\{1,2,...,p\}$ for which there is a $d\times p$ matrix $B_1$ such 
\begin{equation}\label{e:model-vc-ss}
	B_1 A^2(u) B_1' = \Sigma, \; \; \forall \; u\in (0,1],
\end{equation}
where  $A^2(u) = A(u) A(u)'$ , $\Sigma$ does not depend on $u$ and $B_1B_1' = I_d$. \\

\textbf{(b):} We say there exists a (second-order) \textit{stationary subspace} of dimension $d$ for model \eqref{e:model-vc} if $d$ is the largest integer in $\{1,2,...,p\}$ for which there is a $d\times p$ matrix $B_1$ such 
\begin{equation*} 
	B_1 A(u)  = W, \; \; \forall \; u\in (0,1], 
\end{equation*}
where the $d \times p$ matrix $W$ does not depend on u and $B_1B_1^{'}=I_d$.
\end{definition}

Note that definition (b) implies $B_1 A^2(u) B_1' = WW^{'} = \Sigma $ which leads to (a) but definition (a) does not imply (b). The latter is because $B_1A(u)$ is a rectangular matrix and there need not exist a decomposition $\Sigma = WW^{'}$ where $W$ is rectangular. In addition, definition (a) is a condition only on the time-invariance of the second moment of $B_1X_t$ whereas definition (b) is a stronger condition involving  time invariance of all moments of $B_1X_t$. \\



Let $\overline{A}^2 = \int_0^1 A^2(u) du$ and define $p \times p$ symmetric matrix $M_u$ as 
\begin{equation} \label{e:models-M}
M_u = A^2(u) - \overline{A}^2.
\end{equation}
  Then the condition in (\ref{e:model-vc-ss}) is equivalent to
\begin{equation}\label{e:model-vc-ss-2}
	B_1 M_u  B_1'  = 0, \; \; \forall \; u \in (0,1].
\end{equation}
From \eqref{e:model-vc-ss-2} we note that the dimension $d$ is related to rank properties of the symmetric matrix $M_u$. In the next section, we take a closer look at these properties. \\

Analogous to \eqref{e:model-vc-ss-2}, we have the following condition equivalent to Definition 2.1 (b)
\begin{equation*}
B_1 (A(u) - \bar{A}) = 0, \; \; \forall u \in (0,1] \;\;\;\;\; 
\end{equation*}
where  $\bar{A} = \int_{0}^1 A(u)du$. \\

\begin{remark}\label{r:ssa-formulations}
We note that the relation (\ref{e:model-vc-ss-2}) is not the only way to reformulate the condition (\ref{e:model-vc-ss}). For example, the following conditions are also equivalent to (\ref{e:model-vc-ss}): 
\begin{equation}\label{e:model-vc-ss-3}
	B_1 \Big(A^2(u)  -  \frac{1}{c_2- c_1}\int_{c_1}^{c_2} A^2(u)du \Big) B_1'  = 0, \; \; \forall \; u\in (0,1],
\end{equation}
for fixed $0<c_1<c_2<1$. The choices of $c_1$ and $c_2$ while estimating $M_u$ in finite sample cases is further discussed in Section \ref{s:simulation_dimension}.

%, or 
%\begin{equation}\label{e:model-vc-ss-4}
%	B_1 \Big(A^2(u)  -  A^2(u_0)  \Big) B_1'  = 0,\quad u\in %(0,1],
%\end{equation}
%where $u_0\in(0,1]$ is fixed. 
%The role of these various formulations remains to be clarified from the practical standpoint. In this work, we shall use (\ref{e:model-vc-ss-2}) and sometimes (\ref{e:model-vc-ss-3}), the latter when the analysis is on a subinterval of $(0,1]$.
\end{remark}


